CoDream: Exchanging dreams instead of models for federated aggregation with heterogeneous models

Federated Learning (FL) enables collaborative optimization of machine learning models across decentralized data by aggregating model parameters. Our approach extends this concept by aggregating "knowledge" derived from models, instead of model parameters. We present a novel framework called CoDream, where clients collaboratively optimize randomly initialized data using federated optimization in the input data space, similar to how randomly initialized model parameters are optimized in FL. Our key insight is that jointly optimizing this data can effectively capture the properties of the global data distribution. Sharing knowledge in data space offers numerous benefits: (1) model-agnostic collaborative learning, i.e., different clients can have different model architectures; (2) communication that is independent of the model size, eliminating scalability concerns with model parameters; (3) compatibility with secure aggregation, thus preserving the privacy benefits of federated learning; (4) allowing of adaptive optimization of knowledge shared for personalized learning. We empirically validate CoDream on standard FL tasks, demonstrating competitive performance despite not sharing model parameters. Our code: https://mitmedialab.github.io/codream.github.io/

==> neurips/preamble.tex <==
\DeclareRobustCommand{\abhi}[1]{ {\begingroup\sethlcolor{orange}\hl{(abhi:) #1}\endgroup} }
\DeclareRobustCommand{\charlie}[1]{ {\begingroup\sethlcolor{cyan}\hl{(charlie:) #1}\endgroup} }
% \DeclareRobustCommand{\rchi}{{\mathpalette\irchi\relax}}
% \newcommand{\irchi}[2]{\raisebox{\depth}{$#1\chi$}} % inner command, used by \rchi
\newcommand{\rchi}{\mathcal{X}}
\newcommand{\data}{\mathcal{D}}
\newcommand{\batch}{\hat{x}}
\newcommand{\keloss}{\tilde{\ell}}
\newcommand{\collabkeloss}{\phi}
\newcommand{\client}{k}
\newcommand{\clients}{K}
\newcommand{\kl}{\mathsf{KL}}
\newcommand{\ce}{\mathsf{CE}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\newcommand{\expectation}{\mathop{\mathbb{E}}}

\usepackage{xspace}
\newcommand{\codream}{\texttt{Co-Dream}\xspace}
\newcommand{\feddream}{\texttt{Co-Dream}\xspace}
\newcommand{\fedavg}{\texttt{FedAvg}\xspace}
\newcommand{\fedprox}{\texttt{FedProx}\xspace}
\newcommand{\scaffold}{\texttt{SCAFFOLD}\xspace}
\newcommand{\moon}{\texttt{MOON}\xspace}
\newcommand{\akd}{\texttt{AKD}\xspace}
\newcommand{\ekd}{\texttt{AKD}\xspace}
\newcommand{\fedgen}{\texttt{FedGen}\xspace}
\newcommand{\independent}{\texttt{Independent}\xspace}
\newcommand{\centralized}{\texttt{Centralized}\xspace}

==> sec/old_0_intro.tex <==
https://www.overleaf.com/project/63e3b59505e299d0d6d34f42

\section{Introduction}
% Context; An introduction to the problem sphere; Teaser of our solution
Centralizing data to apply machine learning (ML) in applications such as healthcare, finance, and mobility can be problematic due to regulatory and privacy concerns. Federated learning (FL) offers a potential solution by collaboratively training ML models without centralizing private data. Typically, this is achieved by locally training the model and sharing the model updates with the server that averages these updates. This approach is practical for collaborative training when all the clients share the same model architecture. However, such an assumption could be too restrictive when we need collaboration among clients with different computational resources. Furthermore, with the current trend of billion-parameters models, there is a need for collaborative learning techniques where communication does not scale with the model's size. In this work, we propose an alternate paradigm for FL where updates happen in the data space. Since data dimensionality remains the same across clients, our approach avoids issues related to different model architecture and scalability, making our technique model-agnostic and suitable for large-scale models.

% Develop intuition and a high-level solution
Our goal is to provide clients with the flexibility to use any model of their choice while still enjoying the privacy benefits of Federated Learning. The task is challenging because FL algorithms aggregate model updates to improve a common global model. Our main insight is that while model architectures may differ, clients typically have data with the same dimensionality. By sharing knowledge in the data space rather than the model parameter space, clients can use different models for the same task.
FL is amenable to privacy for two reasons - 1) the clients share the model updates instead of raw data, and 2) the clients do not have to reveal their individual local model updates to the server as they can securely (using cryptographic techniques) aggregate their model updates. The second property strengthens privacy as we increase the number of clients.



% More technical solution
Our technique is inspired by Deepdream~\cite{mordvintsev2015inceptionism} that shows features learned by an ML model can be \textit{extracted} using gradient-based optimization in the feature space. We propose \feddream, which takes the idea of gradient-based optimization for extracting knowledge in a federated setting. Once the knowledge is collaboratively extracted from the client models, we utilize knowledge distillation (KD) to integrate the knowledge into the client models. Our approach can be of independent interest as a joint optimization problem in the input space.

% Differentiate
% - Talk succinctly about how to think about existing attempts at model agnostic federated learning, why they are doomed to not work
% - Mention the secure averaging aspect
Several recent works have integrated KD in FL motivated by the concerns around communication efficiency~\cite{jeong2018communication}, data heterogeneity~\cite{zhu2021data}, and model heterogeneity~\cite{afonin2022towards} with \fedavg. The main focus of our work is model heterogeneity where existing works either use publicly available data~\cite{chang2019cronus} or they alter~\cite{li2021decentralized,afonin2022towards} the collaboration algorithm in a way that is incompatible with secure aggregation. However, as discussed before, FL is amenable to privacy because not only do clients share the model parameters, but the individual client updates can also be hidden by secure aggregation. To the best of our knowledge, our framework takes the first steps to retain both privacy benefits of FL while enabling model heterogeneity. As we discuss later in Sec~\ref{sec:method-benefits} and show experimentally~\ref{sec:expts}, our approach also yields benefits in communication and data heterogeneity. Existing works alleviating data heterogeneity, such as \fedprox~\cite{sahu2018convergence}, \scaffold~\cite{karimireddy2020scaffold}, and \moon~\cite{} can be viewed as adjacent works that can be utilized to improve the quality of federated averaging in the feature space proposed in our work.
% - Co-distillation types: Avg not possible
% - FedDistill, Fred's work: Only aggregated output is shared and hence not enough signal is present
% - Require public data:
% - Server based generative model learning: The clients do not contribute in learning the data representation
\begin{figure}
    \centering
    \includegraphics[width=0.7\columnwidth]{figs/teaser_p3_1.png}
    \caption{Existing Federated Learning techniques perform a linear aggregation that allows using secure aggregation of local client updates but requires the same model architecture across users. While knowledge distillation offers a model-agnostic knowledge transfer, it currently does not support secure aggregation. We enable linear and model-agnostic aggregation by aggregating gradients in the input space. \abhi{change the title in the diagram}}
    \label{fig:my_label}
\end{figure}

% Define the scope for privacy and malicious behavior
\textbf{Scope of the paper} - Our primary focus is on validating the collaborative learning aspect of our work, specifically the design of the \feddream algorithm. While \feddream is designed to be privacy-preserving similarly to \fedavg in the parameter space, our investigation does not extensively address privacy or robust aggregation mechanisms. We do, however, note that our knowledge extraction procedure begins with random input and is optimized using gradients from an ML model, which implies that the mutual information between the shared knowledge and the raw data is lower than the mutual information between the data and the model, as per the post-processing inequality. This reduction in mutual information between the raw data and the shared knowledge has the potential to be leveraged for designing mechanisms that achieve a favorable privacy-utility trade-off, but we leave this as future work. Similarly, \feddream can be used in conjunction with robust averaging techniques to improve the performance of FL frameworks in the presence of malicious clients, as the low dimensionality of the vector to be aggregated is achieved through knowledge sharing in the input space rather than the parameter space.

% Summarize
% For contributions - what is the precise contribution and why is it a contribution (why is it both novel and useful).
We design our framework into three stages - 1) Knowledge extraction~\ref{sec:method:k-ex}, 2) Knowledge aggregation~\ref{sec:method:k-ag}, and 3) Knowledge acquisition~\ref{sec:method:k-ac}. We quantitatively and qualitatively investigate~\ref{sec:expts} the feasibility of \feddream as a competitive alternative to existing FL frameworks across commonly benchmarked (IID and non-IID) settings and datasets, i.e. i) MNIST~\cite{lecun1998gradient}, ii) EMNIST~\cite{cohen2017emnist}, and iii) CIFAR10~\cite{krizhevsky2009learning} as well as a medical imaging dataset PathMNIST~\cite{yang2023medmnist}. Our experiments resulted in several intriguing observations about the federated optimization in the input space that, to the best of our knowledge, have not been studied before and could be of independent interest. Our contributions are summarized as follows:
\begin{itemize}
    \item A framework for model agnostic Federated Learning by optimization in the input space. Similar to \fedavg, the synchronization step between the clients is a linear operation (weighted average) and is hence amenable to secure aggregation.
    \item We formulate the learning of a global model as a knowledge acquisition problem and design a personalized distillation procedure for \textit{adaptively} extracting knowledge from the clients. Our personalized distillation technique can be applied for personalized FL.
    \item Empirical validation by benchmarking with existing algorithms and ablation studies across various design choices.
\end{itemize}

%  Our main contributions are summarized as follows:
%The paragraphs below need to be in the Method Section
% Plenty of  
% A little primer Why is the problem challenging
% The main intuition behind applying KD for FL is to treat each client as a teacher and use their output as a surrogate source of ground truth. Then, all other participants in the system can be treated as students (the server could also aggregate knowledge from all teachers by ensembling their outputs). KD effectively transfers knowledge because these ``soft-logits'' capture semantic relationships between different classes. For example, a model fed a dog image with cat-like features will produce a higher score for the cat logit than non-cat classes such as chair or car. Since most datasets share such hierarchical relationships, the student can learn those by mimicking the input-output of an expert model. However, to exploit these relationships, the student needs access to datasets over which the teacher can capture such semantic relationships. This requirement explains why KD cannot be applied naively to federated learning because a client wants to learn from other experts but does not have access to their datasets and, therefore cannot benefit from their soft logits. This intuition is formally demonstrated by the negative result from \citet{afonin2022towards}. While KD is a promising model-agnostic alternative to traditional federated learning model aggregation, its need for access to teacher distribution is against the spirit of collaborative ML over decentralized data. To address this dilemma, we design a (model agnostic) algorithm that \textit{collaboratively} learns the input space from all users (teachers).


% Insights and Differentiate
% Our key insight is that a reasonable representation of local datasets can be obtained by simply querying the ML models trained on them. DeepDream~\cite{mordvintsev2015inceptionism} demonstrates we can extract patterns learned by a trained neural network (NN) by optimizing a randomly initialized feature to maximize particular activation maps of the NN. DeepInversion~\cite{yin2020dreaming} further improves this knowledge extraction process by utilizing the batch norm statistics stored in the layers of the NN. Such an extracted dataset can be used to represent the samples from a user. While a similar principle is used in some of the model inversion attacks, our approach to obtaining representations from models is tailored for collaborative learning instead. Existing approaches have performed \textit{data-free} knowledge distillation by either using public datasets or learning a generative data model. Our approach can be viewed as learning a generative model of data. However, we perform optimization in the data space, enabling secure aggregation over the server while staying model agnostic.

% Our main contribution is a collaborative optimization algorithm where clients optimize the representation of their data distribution locally and share the updates with the server for aggregation. For every client, the optimization starts with a random feature and updates the feature with respect to model weights to maximize the model's \textit{confidence} over that feature. The aggregated updates by the server can be viewed as a representation of different clients' data distribution. Similar to FL (and data parallel distributed machine learning generally), there are multiple rounds of local optimization steps and synchronization rounds of local updates. Unlike FL, the optimization happens in the data space, not the parameter space. Optimization in data space makes our approach model agnostic. The collaborative approach of our framework, i.e. aggregation of gradients in the data space, means secure aggregation~\cite{bonawitz2017practical} can be utilized for securely aggregating updates over many clients. Using gradient-based optimization allows for incorporating additional objectives in generating the representation. For instance, we demonstrate how our framework enables clients to \textit{learn} what they do not \textit{know}, and others do. Specifically, a given client can obtain representations that they are not \textit{confident} about, but others are. Hence, they can use such a representation and its expert output to improve their model.

% Clearly define the scope, no confusion after this point
% \textbf{Note on Privacy} -  The privacy of raw data is protected at two stages in FL. First, sharing an ML model instead of raw data with the server brings an informal sense of privacy.  In the worst case, an attacker can successfully approximate the weights of a target user. Therefore, existing defense mechanisms for preventing leakage from weights are applicable here too. Second, secure aggregation~\cite{bonawitz2017practical} can be utilized to reveal the aggregated model weights to the untrusted server. Secure aggregation is computationally inexpensive due to the linearity of the aggregation process. Our framework also utilizes a linear aggregation of local updates from all clients and is amenable to secure aggregation techniques. We note that both stages do not guarantee full privacy therefore, they are additionally augmented with a differentially private (DP) mechanism. In theory, it is possible to design new mechanisms for our knowledge extraction query with a better privacy-utility trade-off than privatizing the model updates; however, we leave it for future work.


% \textbf{Scope for malicious behavior} - We assume honest but curious users; therefore, a teacher is not expected to harm other students' models in our current design maliciously. Our goal is to develop the collaborative learning framework; therefore, we leave the study and design of the robustness of the proposed framework as part of future work.


==> sec/old_1_rw.tex <==
\section{Related Work}
% The goal of integrating KD into FL is based on several motivations, such as data heterogeneity, model heterogeneity, and communication efficiency. We refer the reader to \cite{mora2022knowledge} for a comprehensive survey. 
From the perspective of our paper, existing works can be categorized based on two characteristics: how knowledge is extracted from the teachers and how the students aggregate and acquire the teachers' knowledge.

\textbf{Knowledge extraction}: One of the key components of KD is to match the output distribution between the teacher and the student conditioned on the same input. Therefore, the same input is needed between the teacher and the student. However, FL techniques typically assume that the student and the teacher have different data siloes. This constraint has led to two general approaches to KD-based FL:
\begin{itemize}
    \item \textbf{Proxy data-based} techniques assume publicly available datasets to obtain the output distribution among different users. Cronus~\cite{chang2019cronus}, Federated model fusion~\cite{lin2020ensemble},\abhi{add more public data based citations} and FedBE~\cite{chen2021fedbe}. Instead of relying on a publicly available dataset, \cite{afonin2022towards} utilize the student's dataset to obtain the teacher's predictions by exchanging the teacher's model. A general drawback of these approaches is that the proxy dataset has to be a sufficiently rich representation of the original data distribution to enable knowledge sharing, which can be an overly constraining assumption for FL.
    \item \textbf{Data Free} techniques learn a generative data model. DENSE~\cite{zhang2022dense}, Fedgen~\cite{zhu2021data}, and FedFTG~\cite{zhang2022fine} learn a generative model of data on the server. While not focused on knowledge distillation, dataset distillation techniques such as Fed-D3~\cite{song2022federated} and DOS-FL~\cite{zhou2020distilled} perform dataset distillation locally and share the distilled datasets with the server, where a global model is trained with one-shot communication. \cite{jeong2018communication} and \cite{berdoz2022scalable} aggregate the last layer's output on the private data across different samples for every class. \charlie{mention how this work is different from DENSE}
\end{itemize}
\textbf{Knowledge Acquisition}: The other key component of KD is the alignment between the teacher's and the student's output distribution $\kl(p(f_{\theta_t}(x))||p(f_{\theta_s}(x)))$ is computed and minimized by optimizing the parameters of the student. Existing approaches can be broadly categorized into where this distribution alignment is performed.
\begin{itemize}
    \item \textbf{Client model regularization} - The clients regularize their local model training by treating other clients as teachers. \cite{lee2021preservation} regularizes on all labels concerning the aggregated teacher model except the original label to avoid catastrophic forgetting. \cite{afonin2022towards} perform distillation locally by using the teacher model on the client's data. \cite{zhu2021data} distribute the synthetic data generator learned by the server to the clients for regularization during training.
    \item \textbf{Ensemble distillation} techniques regularize the global server model using proxy or synthetic data. FedBE~\cite{chen2021fedbe}, Ensemble Distillation~\cite{lin2020ensemble}, FedAux~\cite{sattler2021fedaux}, and FedFTG~\cite{zhang2022fine} aggregate soft labels from different clients.
\end{itemize}


Independently of knowledge distillation, a few recent works have accommodated model heterogeneity by sub-model extraction~\cite{caldas2018expanding, diao2021heterofl, th2021fjord,alam2022fedrolex} and factorizing model weights with low-rank approximations~\cite{mei2022resource}. Most of these techniques only support heterogeneity for a specific class of models, for example - the ResNet family. In contrast, KD-based approaches are more flexible and only require the input and output dimensionality to be the same.

==> sec/old_2_method.tex <==
% Preliminaries
% Federated Learning
% Knowledge Distillation
% FedDream
% - K-Ex
% - K-Ag
% - K-Ac
% - Analysis

\begin{table}[]
    \centering
    \includegraphics[width=0.8\textwidth]{tabs/landscape_table.pdf}
    \caption{Landscape of Federated Learning techniques with respect to our work.}
    \label{tab:my_label}
\end{table}

\section{Preliminaries}
\textbf{Federated Learning} (FL) aims to optimize the expected risk $\min_{\theta}\mathbb{E}_{\data\sim p(\data)} \ell(\data, \theta)$ where $\data$ is a tuple of samples $\{X\in\rchi, Y\in\mathcal{Y}\}$ of labeled data in supervised learning in the data space $\rchi\subset\mathbb{R}^d$ and $\mathcal{Y}\subset\mathbb{R}$. $\ell$ is a risk function typically kept as mean square error or cross-entropy for classification tasks. In the absence of access to the true distribution, FL aims to optimize the empirical risk instead, i.e. $\min_{\theta}\sum_{\client\in \clients} \frac{1}{|\data_\client|} \ell(\data_\client, \theta)$. Here each $\data_\client$ is owned by a client $\client$ in the system and $\data$ is assumed to be partitioned across $\clients$ clients, i.e. $\data=\cup_{\client\in\clients} \data_\client$. The optimization proceeds with the server broadcasting $\theta^t$ to each client $k$ that locally optimizes $\theta_k^{t+1}=\argmin_{\theta^t}\ell(\data_\client, \theta^t)$ for $r$ rounds and sending local updates either in the form of $\theta_\client^{t+1}$ or $\theta_\client^{t+1} - \theta_\client^t$ (\textit{pseudo-gradient}) with the server that aggregates these local updates from all the clients and send it back to the clients to repeat the process.

% KD
\textbf{Knowledge Distillation} (KD) facilitates the transfer of "knowledge" from an expert teacher model ($f(\theta_T)$) to a student model ($f(\theta_S)$) by augmenting the student's training objective with an additional regularization term. This regularization term, computed using the Kullback-Leibler (KL) divergence $\kl(f(\theta_T, \data)||f(\theta_S, \data))$, encourages the output distribution of the student model to match that of the teacher model. This alignment of output distributions is meaningful when the knowledge learned by the teacher cannot be acquired by the student model on its own. KD is an attractive alternative to \fedavg and its variants in the context of Federated Learning (FL), as the conceptual goal of FL is also to share knowledge among clients that they cannot learn independently. However, applying KD in the FL setting is not trivial, as the student and teacher models typically need access to the same sample, which may not be feasible in the distributed and privacy-constrained FL setting.
%This situation often arises when the student model has limited capacity in terms of parameters compared to the teacher model. Hence, KD was originally invented~\cite{buciluǎ2006model,hinton2015distilling} and is still widely used for model compression, leveraging supervision from a heavily parameterized teacher to improve the performance of a smaller student model.

\textbf{Data-free KD for FL} approaches have been proposed to address this challenge~\cite{zhang2022dense,zhang2022fine,zhu2021data}, where a generator model is trained by querying the client models and generating samples from it for knowledge transfer. However, a key missing piece in these approaches is the lack of active client collaboration in synthesizing ``knowledge.'' Instead, clients share their local models with the server without actively contributing to the knowledge synthesis process. We believe collaborative synthesis is essential for securely aggregating clients' contributions and bridging the gap between knowledge distillation and Federated Learning (FL). Therefore, we design \feddream to enable clients to synthesize samples while ensuring compatibility with secure aggregation techniques collaboratively.
%Furthermore, the functional view of KD, i.e. matching of output distribution between expert and non-expert, makes it model agnostic enabling several advantages such as FL over heterogeneous models and potentially higher communication efficiency. However, regularizing with the teacher's distribution requires access to the samples from the distribution on which the teacher was trained. This constraint makes applying KD naively to FL challenging because users can not share their samples with each other. Consequently, several works circumvent this issue by relying on publicly accessible datasets. However, for KD to be effective, these public datasets should contain samples that also belong to the teacher's distribution with high likelihood. Therefore, assuming public datasets are accessible can be a highly restrictive assumption for certain applications. This limitation of KD for FL has resulted in data-free KD.

% Data Free KD
% \textbf{Data Free KD} algorithms aim to achieve the same functionality as KD of transferring knowledge from a teacher to a student without requiring access to samples from the teacher's distribution. These algorithms can be broadly split into two categories - 1) synthetic data-based and 2) aggregated data-based. Synthetic data-based techniques typically learn a generative data model either in the image space~\cite{zhang2022dense,zhang2022fine} or feature space~\cite{zhu2021data}.
%Aggregation-based approaches share mean logits for each class from each user that the servers can further aggregate. While aggregation-based approaches~\cite{jeong2018communication, seo202216, berdoz2022scalable} are effective for communication and privacy, their capacity to transfer knowledge is fundamentally limited because only aggregate statistics are shared. Our algorithm can be viewed as.

\section{FedDream}
\label{sec:method}
For designing \feddream, we break down FL into three stages: \textbf{knowledge extraction}, \textbf{knowledge aggregation}, and \textbf{knowledge acquisition}. We first informally describe these three stages and then discuss their technical details in the subsections below.

In the knowledge extraction stage, we aim to obtain useful data representations from each client to benefit the other clients. In the typical parameter averaging-based approach, model updates (weights or pseudo-gradients) can be viewed as learned knowledge that can be extracted from each client. 
In our approach, the clients start with a few warmup rounds to pre-train their local model; afterward, they begin with random noise images that are optimized for two objectives. First, the model should have high \textit{confidence} in its output on the optimized images. Second, the optimized images should be close to the statistics of the original data distribution.

We exploit the linearity of gradients to enable knowledge aggregation since our optimization process is a gradient-based optimization scheme. This results in a distributed-SGD (data-parallel) like optimization. \fedavg extends distributed-SGD by performing multiple local steps before synchronization to improve communication efficiency. We utilize the same idea for improving communication as well. Unlike distributed-SGD and \fedavg, the aggregation step occurs in the input space, hence making our approach model agnostic and compatible with FL setups with heterogeneous client architectures.

Finally, for the knowledge acquisition step, the clients share probabilities scores for each image after the images have been collaboratively optimized. This ensemble of scores is aggregated at the server. Owing to the gradient-based optimization in our framework, we describe an adaptive knowledge extraction scheme that can enhance the student's classification performance by enabling the teacher to extract knowledge for a given student adaptively.

\subsection{Local dreaming for extracting knowledge from a model}
\label{sec:method:k-ex}
% We start with a random
The underlying idea of initializing with random features and optimizing them for a given teacher model was first introduced in DeepDream~\cite{mordvintsev2015inceptionism} to identify patterns that maximize a given activation layer in a neural network. Regularization such as TV-norm and $\ell_1$-norm has been shown to improve the quality of the resulting images. Starting with a randomly initialized input $\batch\sim\mathcal{N}(0, I)$ and label $y$, the optimization objective is
\begin{equation}
    \min_{\batch} \ce(f_\theta(\batch), y) + \mathcal{R}(\batch),
    \label{eq:deepdream}
\end{equation}
where $\ce$ is cross-entropy and $\mathcal{R}(\cdot)$ is a regularizar. 

As shown in the DeepInversion paper~\cite{yin2020dreaming}, the knowledge distillation can be further improved by matching batch normalization statistics:
\begin{equation}
    \mathcal{R}_{bn}(\batch) = \sum_{l}\bigl\|\mu_l(\batch) - \mathbb{E}_\data\bigl[\mu_l(x)\bigr]\bigr\|_2 + \bigl\|\sigma_l(\batch) - \mathbb{E}_\data\bigl[\sigma_l(x)\bigr]\bigr\|_2,
    \label{eq:batchnorm}
\end{equation}
where $x\in\rchi$ are the original samples from a dataset and $\mu_l(\cdot)$ and $\sigma_l(\cdot)$ are mean and variance for the $l$'th layer's feature maps for a given batch. The value $\mathbb{E}_{\data}[\mu_l(x)]$ can be approximated using the running mean and variance of the batch normalization layers stored in a model. While DeepDream and DeepInversion enable data-free knowledge extraction, they are not directly applicable to FL because the teacher models i.e. the clients, are continuously evolving, and the student i.e. the server, is learning from multiple teachers as well as its own data. A direct consequence of this non-stationarity is that it is unclear how $y$ should be chosen in eq~\ref{eq:deepdream}. In DeepInversion, the teacher uniformly samples $y$ from its own label distribution because the underlying assumption is that the teacher has the full dataset. However, we cannot assume this in FL because data is distributed across multiple clients with heterogeneous data distributions. Additionally, any given client should only synthesize those samples over which they are highly confident. The central issue with directly applying Eq~\ref{eq:deepdream} is how to keep track of a given client's confidence. We take a simple approach of treating the entropy of the output distribution as a proxy for the teachers' confidence. We adjust Eq~\ref{eq:deepdream} such that the teacher synthesizes the representations without any classification loss and minimizes the entropy (denoted by $\mathcal{H}(\cdot)$) of the output distribution instead. More formally, we optimize the following objective for synthesizing representations -
\begin{equation}
    \label{eq:knowledge_extraction}
    \min_{\batch} \left\{\tilde{\ell}(\batch, \theta):=\mathcal{H}(f_{\theta}(\batch)) + \mathcal{R}(\batch)\right\}.
\end{equation}

A teacher starts with a batch of representations sampled from a standard Gaussian ($x=\mathcal{N}(0, 1)$). The samples are optimized using Eq~\ref{eq:knowledge_extraction}. As opposed to Eq~\ref{eq:deepdream}, we do not restrict $\batch$ in the input space of a neural network but rather allow it to be any representation at a given layer. In Sec~\ref{sec:expts}, we show that for certain experimental setups, sharing representations from the penultimate layer performs equally well as sharing data in the input space. Note that, unlike generative models, the only goal of optimizing these images is to enable knowledge distillation rather than maximize the likelihood of the data. Therefore, the images do not need to appear like a real image. We show several visual results for image datasets in Sec~\ref{sec:expts}.

\subsection{Collaborative dreaming for knowledge aggregation}
\label{sec:method:k-ag}
For a moment, let us assume the server is trusted. The best way to aggregate knowledge would be to aggregate the raw data from all clients at the server, train a teacher model on this aggregated dataset, and apply the knowledge extraction objective described in Eq~\ref{eq:knowledge_extraction}. This can be written as 

\begin{equation}
  \min_{\batch}\tilde{\ell}\left(\batch,\theta^*\right) \;\;\text{s.t.}\;\; \theta^* = \argmin_{\theta}\expectation_{\data_k\sim p(\data)}\left[\ell\left(\data_k, \theta\right)\right].
  \label{eq:centralized_ke}
\end{equation}
However, without centralized data or models, we can not obtain $\theta^*$. Furthermore, estimating $\theta^*$ using $\fedavg$ will not be model-agnostic. Therefore, we collaboratively optimize the representations by taking the expectation over every client's own loss with respect to the same $\batch$:

\begin{equation}
  \min_{\batch}\expectation_{\data_k\sim p(\data)}\left[\collabkeloss(\batch,\data_k):= \keloss\left(\batch, \argmin_{\theta}\ell\left(\theta, \data_k\right)\right)\right].
  \label{eq:distrib_ke}
\end{equation}

Eq~\ref{eq:distrib_ke} can be optimized for distributed data even if it is not equivalent to optimizing the Eq~\ref{eq:centralized_ke}. The empirical risk corresponding to Eq~\ref{eq:distrib_ke} can be minimized by computing local loss at each client. Therefore, the update rule for $\batch$ can be written as
$$\batch \leftarrow \batch - \nabla_{\batch}\sum_{\data_k\in\data}\frac{1}{|\data_k|}\collabkeloss\left(\batch, \data_k\right).$$

While no single party can compute this gradient because models are decentralized due to the linearity of gradients, we can write the above equation as -
\begin{equation}
    \batch \leftarrow \batch - \sum_{\data_k\in\data}\frac{1}{|\data_k|}\nabla_{\batch}\collabkeloss\left(\batch, \data_k\right)
    \label{eq:fedream}
\end{equation} 

Based on the above update rule, the clients can compute gradients locally with respect to the input and share it with the server that aggregates the gradients and sends the updated input back to the clients. Note that this formulation is the same as the distributed-SGD formulation, except the parameters getting optimized are in the input space instead of the model parameter space. Due to the linearity of the aggregation step, it is compatible with cryptographic aggregation techniques that only reveal the final output of the aggregation and not individual clients' gradients. To the best of our knowledge, the idea of collaboratively optimizing representations is not explored before. It is not intuitive why averaging the gradients from different clients will lead to any reasonable representations. However, to our surprise, not only did we find that representations obtained via this approach capture knowledge from all the clients, but they are also more effective representations (as measured by the student's i.e. server's performance) than the ones synthesized by different clients independently. While we investigate this phenomenon in Sec~\ref{sec:expts}, we believe a more comprehensive study of this approach will be of independent interest to the community.

Like how \fedavg extends distributed-SGD by performing multiple gradient descent steps locally on the client device, we extend the Eq~\ref{eq:fedream} to allow multiple local updates. Therefore, the optimization proceeds as follows -

1) At the start of every round $r$, each client $k$ starts with the same parameter $\batch^r_{k, 0} := \batch^{r-1}$ and update its local parameters for $M$ steps, i.e., $$\batch^r_{k, m} = \batch^r_{k, m-1} - \eta_l g_k(\batch^r_{k, m-1})$$

Here, $g_k(x) := \nabla_x(\keloss(x, \data_k))$ is gradient function for the client $k$ and $\eta_l$ is the local learning rate for the clients. Upon the completion of the local optimization, each client sends its local updates $\batch^r_{k, M} - \batch^r$ to the server. The local updates are commonly referred to as pseudo-gradients and are aggregated by the server as follows -
$$\batch^{r+1} = \batch^r + \eta_g \sum_{k \leq K}\frac{1}{\left|\data_k\right|} \left(\batch^r_{k, M} - \batch^{r}\right)$$
Note that the choice of parameters such as local updates $M$, local learning rate $\eta_l$, global rate $\eta_g$, and the number of clients $K$ typically guide the trade-off between communication efficiency and convergence of the optimization problem. We leave the convergence analysis for our algorithm as part of future work and focus primarily on empirical evaluation.

\subsection{Knowledge Acquisition with adaptive teaching}
\label{sec:method:k-ac}
So far, we have discussed how clients can collaboratively extract knowledge from their local models. Now we discuss how to acquire this extracted knowledge in the local models. \abhi{discuss ensembling of logits in detail here}. 

We train the server model using a typical knowledge distillation procedure where the server learns to match the distribution of the ensemble of clients on the dataset of distilled samples (denoted by $\hat{\data_S}$) obtained via solving Eq~\ref{eq:distrib_ke}. Specifically, the server optimizes the following objective:
\begin{equation}
    \min_{\theta_s}\sum_{\batch\in\hat{\data_S}}\kl\left(\sum_k\frac{1}{|\data_k|}f_{\theta_k}(\batch)\bigg\|f_{\theta_S}(\batch)\right).
\end{equation} 

The clients can now train on knowledge from the server, which is $\{\batch, f_{\theta_S}(x) | \batch\in\hat{\data_S}\}$, as its training dataset and perform standard supervised learning, where the server is the teacher and the client act as the student. We call this mode passive knowledge transfer. In passive knowledge transfer, the student does not influence how the teacher extracts knowledge. 

However, by personalizing a student's teaching by what they do not know and what the teacher knows, we can improve the student's performance and make learning faster. The teacher can synthesize examples that maximize the student's loss thanks to gradient-based optimization. The student, in turn, can optimize its model weights to minimize its loss.  Additionally, by personalizing the student's learning, the teacher avoids extracting redundant knowledge. For instance, a student who is trained only on dogs and wants to learn a classification rule for dogs and cats can benefit vastly from getting trained on cat images. The problem is not specific to the difference in the label distribution but in the feature distribution more generally (cats with furs more than other kinds of cats, for example). 

In our framework, we introduce adaptive teaching at two levels. We first adaptively train the server to accelerate its learning. Once the server has compressed the knowledge from different clients into its own model, the clients learn from the server in the same adaptive manner. Now we illustrate our adaptive teaching framework in detail in a single teacher and a single student framework and then extend it to apply under our framework for the server and clients.

\textbf{Adaptive Teaching}: For a given sample $\batch$, this adaptive optimization can be performed by solving the following min-max optimization problem
\begin{equation}
    \min_{\batch}\keloss(\batch, \theta_T) - \keloss(\batch, \theta_S)
\end{equation}
Owing to the optimization in the input space, both the teacher and the student can collaboratively minimize this loss without sharing their model with each other as follows -
\begin{equation}
    \batch \leftarrow \batch - \nabla_{\batch}  \keloss(\batch, \theta_T) + \nabla_{\batch} \keloss(\batch, \theta_S)
    \label{eq:adaptive_update}
\end{equation}
Intuitively, a given teacher, by maximizing students' entropy and minimizing its own, is essentially generating representations of what it knows and the student does not. We apply this adaptive teaching technique to the server and the clients in \feddream.

\textbf{Adaptive knowledge acquisition by the server}
Under this setup, the clients operate as adaptive teachers for the server and minimize their loss while maximizing the loss with respect to the server. Specifically, now $\hat{\data_S}$ is obtained by clients collaboratively optimizing the loss (a modification of Eq \ref{eq:distrib_ke})

\begin{equation}
    \min_{\batch}\expectation_{\data_k\sim p(\data)}\left[\collabkeloss(\batch,\data_k)\right] - \keloss(\batch, \theta_S).
    \label{eq:adaptive_server}
\end{equation}



\textbf{Adaptive knowledge acquisition by the clients}
To improve the client's performance beyond what is attainable via \textit{passive knowledge transfer}, after a specified number of warmup rounds in training the server model, we train the clients on personalized extracted knowledge $\{\batch, f_{\theta_S}(x) | \batch\in\hat{\data_k}\}$ which is obtained by
performing a similar adaptive training where the server now takes the role of a teacher and the clients take the role of a student. For a given client $k\in\{1...K\}$, the server and the client optimizes the following objective:

\begin{equation}
    \min_{\batch} \keloss(\batch, \theta_S) - \keloss(\batch, \theta_k).
    \label{eq:adaptive-client}
\end{equation}

The server's knowledge can be viewed as the culmination of all the clients' knowledge into a single model. 
Such knowledge sharing can be mediated among clients by performing a peer-to-peer information exchange. However, the communication complexity will grow quadratically with respect to the number of clients in the system. In contrast, a server-based system shrinks that communication complexity to constant time with respect to the number of clients because each client only needs to exchange information with the server now and the server's communication increases linearly with the number of clients.
% The idea of flipping the gradients for learning what you don't know
% The server acquires knowledge by adding negative gradients in the first phase, upon the server's convergence
% The clients will learn adaptively by performing gradient aggregation

% Show the results first.
% [Assumption] talk about the adaptive knowledge acquisition

% Give the framework end-to-end
%     - How is the knowledge incorporated?
% Bring in the privacy argument
%    - At least as private as sharing the model weights
%    - Applicable for secure averaging by clients
\subsection{Analysis of \feddream}
\label{sec:method-benefits}
\textbf{Communication Comparison} - For understanding the communication efficiency of this procedure - let us recall our notations where inputs are of dimension $d$, number of samples $n$ to generate, and number of aggregation rounds as $R$. Since our approach is model agnostic, the total communication size is of the order $d\times n\times R$. In FedAvg and its recent variants, the communication size is usually of the order $|\theta|\times R$. For heavily parameterized models currently used in deep learning $|\theta| \ll d\times n$. We comprehensively evaluate the role of $n$ in the system's performance.

\paragraph{Benefits} of \feddream are inherited from the usage of knowledge distillation, along with additional advantages arising from our specific optimization technique.\\
\textbf{Low data dimensionality:} \feddream communicates input gradients ($\nabla_{\batch}$) instead of model gradients ($\nabla_\theta$), which can be advantageous for robust averaging and privacy mechanisms due to their dependence on the dimensionality of samples for their trade-offs. Moreover, the data dimensionality remains constant even if the neural networks increase in depth and width, making this approach suitable for large foundational models in Federated Learning.\\
\textbf{Optimization in the input space:} offers significant flexibility. First, it is model agnostic, allowing for client collaboration with different ML models. Second, the shared input is interpretable, enabling better understanding and analysis of the learned knowledge. Third, clients can collaborate without revealing their proprietary ML models, enhancing privacy. Fourth, sharing knowledge in the input space enables adaptive optimization, such as synthesizing adversarially robust samples or class-conditional samples. Finally, the linearity of the aggregation algorithm makes our approach compatible with secure averaging~\cite{bonawitz2017practical}.

\paragraph{Limitations} of \feddream are mainly due to the additional layer of optimization for distilling representations, i.e. the clients now need to optimize ML models locally and optimize representations collaboratively. Therefore, the following limitations arise -\\
\textbf{Additional computation on the client device:} While the number of parameters on the client device remains unchanged, as gradients are applied in the input space, there is an additional computation burden on the client device. This additional computation can be offloaded to the server if secure aggregation is not required.\\
\textbf{Sample inefficient} - Experimentally, we find that a high number of samples is required for effectively transferring knowledge among clients due to the redundancy of features in independently generated $\batch$. We believe the problem can be circumvented by not using the same initialization, and we show promising results in Sec~\ref{sec:expts}.

\textbf{Scope of the paper} - Our primary focus is on validating the collaborative learning aspect of our work, specifically the design of the \feddream algorithm. While \feddream is designed to be privacy-preserving in a similar manner to \fedavg in the parameter space, our investigation does not extensively address privacy or robust aggregation mechanisms. We do, however, note that our knowledge extraction procedure begins with random input and is optimized using gradients from an ML model, which implies that the mutual information between the shared knowledge and the raw data is lower than the mutual information between the data and the model, as per the post-processing inequality. This reduction in mutual information between the raw data and the shared knowledge has the potential to be leveraged for designing mechanisms that achieve a favorable privacy-utility trade-off, but we leave this as future work. Similarly, \feddream can be used in conjunction with robust averaging techniques to improve the performance of FL frameworks in the presence of malicious clients, as the low dimensionality of the vector to be aggregated is achieved through knowledge sharing in the input space rather than the parameter space.

==> tabs/niid_eval.tex <==
\begin{table*}[htb!]
    \begin{center}
        \scalebox{0.8}{
            \begin{tabular}{llccccc|cccc}
                \toprule 
\multicolumn{1}{l}{}  &  & \multicolumn{8}{c}{\textbf{Test Accuracy}}  \\ \hline 
%
Dataset  
&  
Setting 
& \multicolumn{1}{c}{Independent} 
%
& \multicolumn{1}{c}{\fedavg} 
%
& \multicolumn{1}{c}{\fedprox}
%
& \multicolumn{1}{c}{\scaffold}
%
& \multicolumn{1}{c}{\moon}
%
& \multicolumn{1}{c}{FedGen} 
%
& \multicolumn{1}{c}{AKD} 
%
& \multicolumn{1}{c}{\feddream} \\ \hline
%
\multirow{3}{*}{{\begin{tabular}[c]{@{}c@{}}MNIST\end{tabular}}} 
            &$\alpha$ = 0.1 & a & b & c  & d & e & f & g & i\\
            &$\alpha$ = 1 & a & b & c  & d & e & f & g & i\\
            &$\alpha$ = 10 & a & b & c  & d & e & f & g & i\\
            \midrule

\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}CIFAR-10\end{tabular}} 
 &$\alpha = 0.1$ & a & b & c  & d & e & f & g & i\\
 &$\alpha = 1$ & a & b & c  & d & e & f & g & i\\
 &$\alpha = 10$ & a & b & c  & d & e & f & g & i\\
 \midrule
%

\multirow{4}{*} {\begin{tabular}[c]{@{}c@{}}CIFAR-100\end{tabular}} 
            &$\alpha$ = 0.1 &a & b & c  & d & e & f & g & i\\
            &$\alpha$ = 1 & a & b & c  & d & e & f & g & i\\
            &$\alpha$ = 10 & a & b & c  & d & e & f & g & i\\
            \midrule
\multirow{2}{*} {\begin{tabular}[c]{@{}c@{}}PathMNIST\end{tabular}} 
            &$\alpha=1$  & a & b & c  & d & e & f & g & i\\
            &$\alpha=10$ & a & b & c  & d & e & f & g & i\\
            \midrule
\bottomrule 
\end{tabular}} % scale-box end
\caption{Benchmarking across non-IID scenarios}
\label{tab:niid_bench}
\end{center}
\end{table*}
